Cost free hyper-parameter selection/averaging for Bayesian inverse problems with vanilla and Rao-Blackwellized SMC Samplers

In Bayesian inverse problems, one aims at characterizing the posterior distribution of a set of unknowns, given indirect measurements. For non-linear/non-Gaussian problems, analytic solutions are seldom available: Sequential Monte Carlo samplers offer a powerful tool for approximating complex posteriors, by constructing an auxiliary sequence of densities that smoothly reaches the posterior. Often the posterior depends on a scalar hyper-parameter. In this work, we show that properly designed Sequential Monte Carlo (SMC) samplers naturally provide an approximation of the marginal likelihood associated with this hyper-parameter for free, i.e. at a negligible additional computational cost. The proposed method proceeds by constructing the auxiliary sequence of distributions in such a way that each of them can be interpreted as a posterior distribution corresponding to a different value of the hyper-parameter. This can be exploited to perform selection of the hyper-parameter in Empirical Bayes approaches, as well as averaging across values of the hyper-parameter according to some hyper-prior distribution in Fully Bayesian approaches. For FB approaches, the proposed method has the further benefit of allowing prior sensitivity analysis at a negligible computational cost. In addition, the proposed method exploits particles at all the (relevant) iterations, thus alleviating one of the known limitations of SMC samplers, i.e. the fact that all samples at intermediate iterations are typically discarded. We show numerical results for two distinct cases where the hyper-parameter affects only the likelihood: a toy example, where an SMC sampler is used to approximate the full posterior distribution; and a brain imaging example, where a Rao-Blackwellized SMC sampler is used to approximate the posterior distribution of a subset of parameters in a conditionally linear Gaussian model.

==> bibliography.tex <==
\begin{thebibliography}{9}

@article{del2006sequential,
  title={Sequential {M}onte {C}arlo samplers},
  author={Del Moral, Pierre and Doucet, Arnaud and Jasra, Ajay},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={68},
  number={3},
  pages={411--436},
  year={2006},
  publisher={Wiley Online Library},
  url = {https://doi.org/10.1111/j.1467-9868.2006.00553.x}
}

@article{mackay1992bayesian,
  title={Bayesian interpolation},
  author={MacKay, David JC},
  journal={Neural computation},
  volume={4},
  number={3},
  pages={415--447},
  year={1992},
  publisher={MIT Press}
}

@article{sommariva2014sequential,
  title={Sequential {M}onte {C}arlo samplers for semi-linear inverse problems and application to magnetoencephalography},
  author={Sommariva, Sara and Sorrentino, Alberto},
  journal={Inverse Problems},
  volume={30},
  number={11},
  pages={114020},
  year={2014},
  publisher={IOP Publishing},
  url={https://doi.org/10.1088/0266-5611/30/11/114020}
}

@article{consonni1992conjugate,
  title={Conjugate priors for exponential families having quadratic variance functions},
  author={Consonni, Guido and Veronese, Piero},
  journal={Journal of the American Statistical Association},
  volume={87},
  number={420},
  pages={1123--1127},
  year={1992},
  publisher={Taylor \& Francis Group}
}

@article{green2009reversible,
  title={Reversible jump {MCMC}},
  author={Green, Peter J and Hastie, David I},
  journal={Genetics},
  volume={155},
  number={3},
  pages={1391--1403},
  year={2009},
  publisher={Citeseer}
}

@book{robert2013monte,
  title={Monte {C}arlo statistical methods},
  author={Robert, Christian and Casella, George},
  year={2013},
  publisher={Springer Science \& Business Media}
}

@article{tierney1996introduction,
  title={Introduction to general state-space {M}arkov chain theory},
  author={Tierney, Luke},
  journal={Markov chain Monte Carlo in practice},
  pages={59--74},
  year={1996}
}

@inproceedings{Sunseri2018OnMO,
  title={On marginals of {G}aussian random vectors},
  author={Isaac Sunseri and A. Alexanderian},
  year={2018}
}

@article{viani2021bayes,
      title={Where {B}ayes tweaks {G}auss: Conditionally {G}aussian priors for stable multi-dipole estimation}, 
      author={Alessandro Viani and Gianvittorio Luria and Harald Bornfleth and Alberto Sorrentino},
      year={2021},
      journal={Inverse Problems and Imaging},
      volume={15},
      number={5},
      url={https://doi.org/10.3934/ipi.2021030}
}

@article{jeremiah2011bayesian,
  title={Bayesian calibration and uncertainty analysis of hydrological models: A comparison of adaptive {M}etropolis and sequential {M}onte {C}arlo samplers},
  author={Jeremiah, Erwin and Sisson, Scott and Marshall, Lucy and Mehrotra, Rajeshwar and Sharma, Ashish},
  journal={Water Resources Research},
  volume={47},
  number={7},
  year={2011},
  publisher={Wiley Online Library}
}

@article{10.1214/07-EJS158,
author = {Y. Fan and D.S. Leslie and M.P. Wand},
title = {{Generalised linear mixed model analysis via sequential {M}onte {C}arlo sampling}},
volume = {2},
journal = {Electronic Journal of Statistics},
number = {none},
publisher = {Institute of Mathematical Statistics and Bernoulli Society},
pages = {916 -- 938},
keywords = {generalised additive models, longitudinal data analysis, Nonparametric regression, sequential Monte Carlo sampler},
year = {2008},
url = {https://doi.org/10.1214/07-EJS158},
}

@article{Sorrentino_2014,
	url = {https://doi.org/10.1088/0266-5611/30/4/045010},
	year = 2014,
	month = {mar},
	publisher = {{IOP} Publishing},
	volume = {30},
	number = {4},
	pages = {045010},
	author = {Alberto Sorrentino and Gianvittorio Luria and Riccardo Aramini},
	title = {Bayesian multi-dipole modelling of a single topography in {MEG} by adaptive sequential {M}onte {C}arlo samplers},
	journal = {Inverse Problems},
}

@article{fragoso2018bayesian,
  title={Bayesian model averaging: A systematic review and conceptual classification},
  author={Fragoso, Tiago M and Bertoli, Wesley and Louzada, Francisco},
  journal={International Statistical Review},
  volume={86},
  number={1},
  pages={1--28},
  year={2018},
  publisher={Wiley Online Library}
}

@article{jasra2007population,
  title={Population-based reversible jump {M}arkov chain {M}onte {C}arlo},
  author={Jasra, Ajay and Stephens, David A and Holmes, Christopher C},
  journal={Biometrika},
  volume={94},
  number={4},
  pages={787--807},
  year={2007},
  publisher={Oxford University Press}
}

@article{sciacchitano2019sparse,
  title={Sparse {B}ayesian imaging of solar flares},
  author={Sciacchitano, Federica and Lugaro, Silvio and Sorrentino, Alberto},
  journal={SIAM Journal on Imaging Sciences},
  volume={12},
  number={1},
  pages={319--343},
  year={2019},
  publisher={SIAM}
}

@article{del2007sequential,
  title={Sequential {M}onte {C}arlo for {B}ayesian computation},
  author={Del Moral, Pierre and Doucet, Arnaud and Jasra, Ajay},
  journal={Bayesian statistics},
  volume={8},
  number={1},
  pages={34},
  year={2007},
  publisher={Oxford University Press Oxford}
}

@article{del2012adaptive,
  title={An adaptive sequential {M}onte {C}arlo method for approximate {B}ayesian computation},
  author={Del Moral, Pierre and Doucet, Arnaud and Jasra, Ajay},
  journal={Statistics and Computing},
  volume={22},
  number={5},
  pages={1009--1020},
  year={2012},
  publisher={Springer}, 
  url = {https://doi.org/10.1007/s11222-011-9271-y}
}

@article{wan2011bayesian,
  title={A {B}ayesian approach to multiscale inverse problems using the sequential {M}onte {C}arlo method},
  author={Wan, Jiang and Zabaras, Nicholas},
  journal={Inverse Problems},
  volume={27},
  number={10},
  pages={105004},
  year={2011},
  publisher={IOP Publishing},
  url = {https://doi.org/10.1088/0266-5611/27/10/105004}
}

@article{nguyen2015efficient,
  title={Efficient sequential {M}onte-{C}arlo samplers for {B}ayesian inference},
  author={Nguyen, Thi Le Thu and Septier, Fran{\c{c}}ois and Peters, Gareth W and Delignon, Yves},
  journal={IEEE Transactions on Signal Processing},
  volume={64},
  number={5},
  pages={1305--1319},
  year={2015},
  publisher={IEEE}
}

@article{murphy2001rao,
  title={Rao-{B}lackwellised particle filtering for dynamic {B}ayesian networks},
  author={Murphy, Kevin and Russell, Stuart},
  booktitle={Sequential Monte Carlo methods in practice},
  pages={499--515},
  year={2001},
  publisher={Springer},
  url={https://doi.org/10.1007/978-1-4757-3437-9_24}
}

@article{deely1981bayes,
  title={Bayes empirical bayes},
  author={Deely, JJ and Lindley, DV},
  journal={Journal of the American Statistical Association},
  volume={76},
  number={376},
  pages={833--841},
  year={1981},
  publisher={Taylor \& Francis}
}

@article{roos2015sensitivity,
  title={Sensitivity analysis for {B}ayesian hierarchical models},
  author={Roos, Ma{\l}gorzata and Martins, Thiago G and Held, Leonhard and Rue, H{\aa}vard},
  journal={Bayesian Analysis},
  volume={10},
  number={2},
  pages={321--349},
  year={2015},
  publisher={International Society for Bayesian Analysis},
  url ={https://doi.org/10.1214/14-BA909}
}

@article{sorrentino2013dynamic,
  title={Dynamic filtering of static dipoles in magnetoencephalography},
  author={Sorrentino, Alberto and Johansen, Adam M and Aston, John AD and Nichols, Thomas E and Kendall, Wilfrid S},
  journal={The Annals of Applied Statistics},
  pages={955--988},
  year={2013},
  url={https://doi.org/10.1214/12-AOAS611}
}

@inproceedings{syed2021parallel,
  title={Parallel tempering on optimized paths},
  author={Syed, Saifuddin and Romaniello, Vittorio and Campbell, Trevor and Bouchard-C{\^o}t{\'e}, Alexandre},
  booktitle={International Conference on Machine Learning},
  pages={10033--10042},
  year={2021},
  organization={PMLR},
  url={https://proceedings.mlr.press/v139/syed21a}
}

@book{chopin2020introduction,
  title={An introduction to sequential {M}onte {C}arlo},
  author={Chopin, Nicolas and Papaspiliopoulos, Omiros},
  year={2020},
  publisher={Springer},
  url = {https://doi.org/10.1007/978-3-030-47845-2}
}


@TechReport{bernton2019schrodinger,
  author = 	 {Espen Bernton and Jeremy Heng and Arnaud Doucet and Pierre E. Jacob},
  title = 	 {Schr\"odinger Bridge Samplers},
  institution =  {ArXiv},
  year = 	 {2019},
  OPTkey = 	 {},
  type =	 {e-print},
  number =	 {1912.13170},
  url = {https://doi.org/10.48550/arXiv.1912.13170}
}


@article{zhou2016toward,
  title={Toward automatic model comparison: an adaptive sequential {M}onte {C}arlo approach},
  author={Zhou, Yan and Johansen, Adam M and Aston, John AD},
  journal={Journal of Computational and Graphical Statistics},
  volume={25},
  number={3},
  pages={701--726},
  year={2016},
  publisher={Taylor \& Francis},
  url={https://doi.org/10.1080/10618600.2015.1060885}
}

@article{everitt2020sequential,
  title={Sequential {M}onte {C}arlo with transformations},
  author={Everitt, Richard G and Culliford, Richard and Medina-Aguayo, Felipe and Wilson, Daniel J},
  journal={Statistics and computing},
  volume={30},
  number={3},
  pages={663--676},
  year={2020},
  publisher={Springer}
}

@article{morita2008determining,
  title={Determining the effective sample size of a parametric prior},
  author={Morita, Satoshi and Thall, Peter F and M{\"u}ller, Peter},
  journal={Biometrics},
  volume={64},
  number={2},
  pages={595--602},
  year={2008},
  publisher={Wiley Online Library}
}

@article{beskos2014error,
  title={Error bounds and normalising constants for sequential {M}onte {C}arlo samplers in high dimensions},
  author={Beskos, Alexandros and Crisan, Dan O and Jasra, Ajay and Whiteley, Nick},
  journal={Advances in Applied Probability},
  volume={46},
  number={1},
  pages={279--306},
  year={2014},
  publisher={Cambridge University Press},
  url = {https://doi.org/10.1239/aap/1396360114}
}

@article{Gramacy2010,
  title={Importance tempering},
  author={Gramacy, Robert and Samworth, Richard and King, Ruth},
  journal={Statistics and Computing},
  volume={20},
  number={1},
  pages={1--7},
  year={2010},
  url={https://doi.org/10.1007/s11222-008-9108-5},
  publisher={Cambridge University Press}
}

@article{7339702,  
    author={Nguyen, Thi Le Thu and Septier, François and Peters, Gareth W. and Delignon, Yves},  
    journal={IEEE Transactions on Signal Processing},   
    title={Efficient Sequential {M}onte {C}arlo Samplers for {B}ayesian Inference},   
    year={2016},  
    volume={64},  
    number={5},  
    pages={1305-1319},  
    url={https://doi.org/10.1109/TSP.2015.2504342}
}

@article{Drovandi2019,  
    author={L. F. South, A. N. Pettitt, C. C. Drovandi},  
    journal={Bayesian Analysis},
    title={Sequential {M}onte {C}arlo Samplers with Independent {M}arkov Chain {M}onte {C}arlo Proposals},
    year={2019},  
    volume={14},  
    number={3},  
    pages={135-143},  
    url={https://doi.org/10.1214/18-BA1129}
}

@article{jasra2011inference,
  title={Inference for L{\'e}vy-driven stochastic volatility models via adaptive sequential Monte Carlo},
  author={Jasra, Ajay and Stephens, David A and Doucet, Arnaud and Tsagaris, Theodoros},
  journal={Scandinavian Journal of Statistics},
  volume={38},
  number={1},
  pages={1--22},
  year={2011},
  publisher={Wiley Online Library}
}

@article{doucet2000sequential,
  title={On sequential {M}onte {C}arlo sampling methods for {B}ayesian filtering},
  author={Doucet, Arnaud and Godsill, Simon and Andrieu, Christophe},
  journal={Statistics and computing},
  volume={10},
  number={3},
  pages={197--208},
  year={2000},
  publisher={Springer}
}

@article{sarkka2012backward,
  title={A backward-simulation based {R}ao-{B}lackwellized particle smoother for conditionally linear Gaussian models},
  author={S{\"a}rkk{\"a}, Simo and Bunch, Pete and Godsill, Simon J},
  journal={IFAC Proceedings Volumes},
  volume={45},
  number={16},
  pages={506--511},
  year={2012},
  publisher={Elsevier}
}
@article{schafer2013sequential,
  title={Sequential {M}onte {C}arlo on large binary sampling spaces},
  author={Sch{\"a}fer, Christian and Chopin, Nicolas},
  journal={Statistics and Computing},
  volume={23},
  number={2},
  pages={163--184},
  year={2013},
  publisher={Springer}
}

@article{beskos2016convergence,
  title={On the convergence of adaptive sequential {M}onte {C}arlo methods},
  author={Beskos, Alexandros and Jasra, Ajay and Kantas, Nikolas and Thiery, Alexandre and others},
  journal={Annals of Applied Probability},
  volume={26},
  number={2},
  pages={1111--1146},
  year={2016},
  publisher={Institute of Mathematical Statistics}
}

@inproceedings{douc2005comparison,
  title={Comparison of resampling schemes for particle filtering},
  author={Douc, Randal and Capp{\'e}, Olivier and Moulines, Eric},
  booktitle={ISPA 2005. Proceedings of the 4th International Symposium on Image and Signal Processing and Analysis, 2005.},
  pages={64--69},
  year={2005},
  organization={IEEE},
  url={https://doi.org/10.1109/ISPA.2005.195385}
}

@article{ulker2010annealed,
  title={Annealed {SMC} samplers for nonparametric {B}ayesian mixture models},
  author={Ulker, Yener and Gunsel, Bilge and Cemgil, A Taylan},
  journal={IEEE Signal Processing Letters},
  volume={18},
  number={1},
  pages={3--6},
  year={2010},
  publisher={IEEE},
  url={https://doi.org/10.1109/LSP.2010.2072919}
}

@article{robert2021rao,
  title={Rao-{B}lackwellization in the {M}arkov chain {M}onte {C}arlo era},
  author={Robert, Christian P and Roberts, Gareth O},
  journal={International Statistical Review},
  year={2021},
  volume={89},
  number={2},
  pages={237-249},
  url={https://doi.org/10.1111/insr.12463}
}

@article{calvetti2020sparse,
  title={Sparse reconstructions from few noisy data: analysis of hierarchical {B}ayesian models with generalized gamma hyperpriors},
  author={Calvetti, Daniela and Pragliola, Monica and Somersalo, Erkki and Strang, Alexander},
  journal={Inverse Problems},
  volume={36},
  number={2},
  pages={025010},
  year={2020},
  publisher={IOP Publishing}
}

@article{calvetti2019brain,
  title={Brain activity mapping from meg data via a hierarchical {B}ayesian algorithm with automatic depth weighting},
  author={Calvetti, Daniela and Pascarella, Annalisa and Pitolli, Francesca and Somersalo, Erkki and Vantaggi, Barbara},
  journal={Brain topography},
  volume={32},
  number={3},
  pages={363--393},
  year={2019},
  publisher={Springer}
}

@article{everitt2017bayesian,
  title={Bayesian model comparison with un-normalised likelihoods},
  author={Everitt, Richard G and Johansen, Adam M and Rowing, Ellen and Evdemon-Hogan, Melina},
  journal={Statistics and Computing},
  volume={27},
  number={2},
  pages={403--422},
  year={2017},
  publisher={Springer}
}

@article{trotta2008bayes,
  title={Bayes in the sky: {B}ayesian inference and model selection in cosmology},
  author={Trotta, Roberto},
  journal={Contemporary Physics},
  volume={49},
  number={2},
  pages={71--104},
  year={2008},
  publisher={Taylor \& Francis}
}

@article{Robert_2009,
   title={Computational methods for {B}ayesian model choice},
   journal={AIP},
   url={https://doi.org/10.1063/1.3275622},
   publisher={AIP},
   author={Robert, C. P. and Wraith, D. and Goggans, Paul M. and Chan, Chun-Yong},
   year={2009}
}

@misc{arampatzis2018langevin,
      title={Langevin Diffusion for Population Based Sampling with an Application in {B}ayesian Inference for Pharmacodynamics}, 
      author={Georgios Arampatzis and Daniel Wälchli and Panagiotis Angelikopoulos and Stephen Wu and Panagiotis Hadjidoukas and Petros Koumoutsakos},
      year={2018},
      eprint={1610.05660},
      archivePrefix={arXiv},
      primaryClass={stat.CO}
}

@article{neal2001annealed,
  title={Annealed importance sampling},
  author={Neal, Radford M},
  journal={Statistics and computing},
  volume={11},
  number={2},
  pages={125--139},
  year={2001},
  publisher={Springer},
  url={https://doi.org/10.1023/A:1008923215028}
}

@book{liu2008monte,
  title={Monte {C}arlo strategies in scientific computing},
  author={Liu, Jun S},
  pages={34--35},
  year={2008},
  publisher={Springer Science \& Business Media},
  url={https://doi.org/10.1007/978-0-387-76371-2}
}

@article{ristic2011metric,
  title={A metric for performance evaluation of multi-target tracking algorithms},
  author={Ristic, Branko and Vo, Ba-Ngu and Clark, Daniel and Vo, Ba-Tuong},
  journal={IEEE Transactions on Signal Processing},
  volume={59},
  number={7},
  pages={3452--3457},
  year={2011},
  publisher={IEEE},
  url={https://doi.org/10.1109/TSP.2011.2140111}
}

@article{RevModPhys.65.413,
  title = {Magnetoencephalography---theory, instrumentation, and applications to noninvasive studies of the working human brain},
  author = {H\"am\"al\"ainen, Matti and Hari, Riitta and Ilmoniemi, Risto J. and Knuutila, Jukka and Lounasmaa, Olli V.},
  journal = {Rev. Mod. Phys.},
  volume = {65},
  issue = {2},
  pages = {413--497},
  numpages = {0},
  year = {1993},
  month = {Apr},
  publisher = {American Physical Society},
  url = {https://doi.org/10.1103/RevModPhys.65.413}
}

@article{stuart2010inverse,
  title={Inverse problems: a {B}ayesian perspective},
  author={Stuart, Andrew M},
  journal={Acta Numerica},
  volume={19},
  pages={451--559},
  year={2010},
  publisher={Cambridge University Press},
  url={https://doi.org/10.1017/S0962492910000061}
}

@Book{good1965estimation,
  author =	 {Good, Irvine J},
  ALTeditor = 	 {},
  title = 	 {The Estimation of Probabilities: An Essay on Modern Bayesian Methods},
  publisher = 	 {MIT Press},
  year = 	 {1965},
  OPTkey = 	 {},
  OPTvolume = 	 {},
  OPTnumber = 	 {},
  OPTseries = 	 {},
  OPTaddress = 	 {},
  OPTedition = 	 {},
  OPTmonth = 	 {},
  OPTnote = 	 {},
  OPTannote = 	 {}
}

@Article{gerber2019negative,
  author = 	 {Gerber, M and Chopin, N and Whiteley, N},
  title = 	 {Negative association, ordering and convergence of resampling methods},
  journal = 	 {Annals of Statistics},
  year = 	 {2019},
  OPTkey = 	 {},
  volume =	 {37},
  number =	 {4},
  pages =	 {2236-2260},
  OPTmonth = 	 {},
  OPTnote = 	 {},
  OPTannote = 	 {},
  url = {https://doi/10.1214/18-AOS1746}
}

@Article{guarniero2017iterated,
  author = 	 {P. Guarniero and A. M. Johansen and A. Lee},
  title = 	 {The Iterated Auxiliary Particle Filter},
  journal =  {Journal of the American Statistical Association},
  OPTkey = 	 {},
  year =	 {2017},
 volume = {112},
 number = {520},
 pages = {1636--1647},
 url = {https://doi/10.1080/01621459.2016.1222291},
 }



\end{thebibliography}


